Industrial Anomaly Detection and Localization Using Weakly-Supervised Residual Transformers

Recent advancements in industrial anomaly detection (AD) have demonstrated that incorporating a small number of anomalous samples during training can significantly enhance accuracy. However, this improvement often comes at the cost of extensive annotation efforts, which are impractical for many real-world applications. In this paper, we introduce a novel framework, Weak}ly-supervised RESidual Transformer (WeakREST), designed to achieve high anomaly detection accuracy while minimizing the reliance on manual annotations. First, we reformulate the pixel-wise anomaly localization task into a block-wise classification problem. Second, we introduce a residual-based feature representation called Positional Fast Anomaly Residuals (PosFAR) which captures anomalous patterns more effectively. To leverage this feature, we adapt the Swin Transformer for enhanced anomaly detection and localization. Additionally, we propose a weak annotation approach, utilizing bounding boxes and image tags to define anomalous regions. This approach establishes a semi-supervised learning context that reduces the dependency on precise pixel-level labels. To further improve the learning process, we develop a novel ResMixMatch algorithm, capable of handling the interplay between weak labels and residual-based representations. On the benchmark dataset MVTec-AD, our method achieves an Average Precision (AP) of $83.0\%$, surpassing the previous best result of $82.7\%$ in the unsupervised setting. In the supervised AD setting, WeakREST attains an AP of $87.6\%$, outperforming the previous best of $86.0\%$. Notably, even when using weaker annotations such as bounding boxes, WeakREST exceeds the performance of leading methods relying on pixel-wise supervision, achieving an AP of $87.1\%$ compared to the prior best of $86.0\%$ on MVTec-AD.

==> method_back.tex <==
\section{Our proposed Method}
\label{sec:method}

\subsection{Overview of the Inference Stage}
\label{subsec:infer}
\begin{figure*}[ht]  
  \centering
\includegraphics [width=0.95\textwidth]{figs/inference.pdf}
\caption{
  The overview of the inference process of WeakREST. Note that all the tensors with a number
  of channels are all shown as matrix for the reason of simplicity. Better view in color. 
}
\label{fig:infer}
\end{figure*}

The overall inference process of our WeakREST algorithm is illustrated in
Figure~\ref{fig:infer}. As it can be seen, there are three stages in the whole process,
\emph{i.e.}, the residual feature generation stage (the green box), the defect
classification process based on a Swin Transformer model (the yellow box) and a optional
post process for object region reweighting (the blue box). 

As mentioned in the introduction part, this work tries to exploit the intermediate
information of the popular patch-matching process, to achieve better AD performance.


\subsection{PosFAR: Fast Anomaly Residuals with P\-osi\-ti\-on Con\-s\-t\-r\-ai\-n\-ts}
\label{subsec:PosFAR}

\subsubsection{Matching Residual for Anomaly Detection}

Mathematically, for a input image $\mathrm{I} \in \hanxiR^{h_{\mathrm{I}} \times
w_{\mathrm{I}} \times 3}$, one can extract deep features as  
\begin{equation}
  \label{equ:extract}
  [\mathbf{f}_1, \mathbf{f}_2, \cdots, \mathbf{f}_M] \gets \mathrm{Flatten} \gets \mathbf{F} =
  \Psi_{\mathrm{CNN}}(\mathrm{I})
\end{equation}
where $\Psi_{\mathrm{CNN}}(\cdot)$ represents a deep network, which is pre-trained on a
large but neutral dataset (ImageNet \cite{russakovsky2015imagenet} for example);
$\mathbf{F} \in \hanxiR^{h_f \times w_f \times d_f}$ denotes the generated deep feature
tensor with $M$ feature vectors ($M = h_f\cdot w_f$); $\mathbf{f}_i \in \hanxiR^{d_f}, i =
1, 2, \cdots,M$ stands for the $i$-th deep feature vector extracted from the tensor
$\mathbf{F}$. 
One then can build the memory ``bank'' of the defect-free training set as 
\begin{equation}
  {\mathcal{B}}_{raw} = \{{\mathbf{f}}^{ref}_{i,j} \in \hanxiR^{d_f} \mid \forall j = 1, \cdots,
  N_{trn}, \forall i = 1, \cdots, M\}
\end{equation}
where $N_{trn}$ denotes the number of training images. ${\mathcal{B}}_{raw}$ contains
$M\cdot N_{trn}$ feature vectors and is usually further down sampled as  
\begin{equation} 
  \label{equ:coreset}
  {\mathcal{B}} = \Psi_{\mathrm{core}}({\mathcal{B}}_{raw}) = \{{\mathbf{f}}^{ref}_t \in
  \hanxiR^{d_f} \mid \forall t = 1, \cdots, T\}
\end{equation}
where $\Psi_{\mathrm{core}}(\cdot)$ represents the ``coreset'' sampling scheme
proposed in \cite{roth2022towards}, and $T \ll M\cdot N_{trn}$ for decreasing the matching
complexity. Then a test patch feature $\mathbf{f}^{tst}_i$ is matched with the reference
features in ${\mathcal{B}}$ as   
\begin{equation}
  \label{equ:pcr}
  t^{\ast} = \hanxiargmin{\forall t = 1, \cdots, T}\|\mathbf{f}^{tst}_i -
  {\mathbf{f}}^{ref}_t\|_{l_2}.
\end{equation}
The corresponding minimal distance $d_i = \|\mathbf{f}^{tst}_i -
{\mathbf{f}}^{ref}_{t^{\ast}}\|_{l_2}$ is usually used to calculate the anomaly score of the
test patch.

In this work, on the other hand, the residual vector of patch-matching, rather than the
Euclidean distance between matched patches, is used as the network input.  This
intermediate information is usually ignored in the majority of related literature
\cite{roth2022towards, kim2022fapm, bae2022image, saiku2022enhancing, zhu2022anomaly,
xie2023pushing}. Formally, our residual feature is defined as 
\begin{equation}
  \mathbf{r}_i = \lceil \text{ABS}(\mathbf{f}^{tst}_i - {\mathbf{f}}^{ref}_{t^{\ast}})
  \rceil^{\theta} \in
  \hanxiR^{d_f},
\end{equation}
where $\text{ABS}(\cdot)$ denotes the function of absolute value, $\lceil \cdot
\rceil^{\theta}$ stands for the element-wise $\theta$-power operation which is introduced to
emphasis the larger elements in the residual vector.

However, the original patch matching suffers from some drawbacks such as the low efficiency and the ignorance of geometric information. We therefore design a more sophisticated patch matching
scheme and term the yielded residual feature ``\textbf{Pos}itional \textbf Fast
\textbf Anomaly \textbf Residuals'' (PosFAR), as introduced in the following subsections. 

\subsubsection{Position Constrained Features}
\label{subsubsec:pcf}
Recently, new evidences show that, the positional information of the comparing patches
could improve the AD performance \cite{bae2022image, gudovskiy2022cflow} mainly because of
the rough alignment of the test images captured in the industrial environment.
Accordingly, we introduce the ``positional embedding'' concept from the literature of
Transformers \cite{dosovitskiyimage,liu2021swin} to the PatchCore algorithm: the original
patch features are aggregated with their positional features encoded in the Transformer
way \cite{he2022masked}. Mathematically, given a patch feature $\mathbf{f}$ defined in Eq.~\ref{equ:extract}, we generate its ``position-constrained '' version as  
\begin{equation}
  \mathbf{p} = \mathbf{f} + \lambda_{\mathrm{P}}\boldsymbol{\eta} =
  \mathbf{f} +\lambda_{\mathrm{P}}\Phi_{\mathrm{P}}(r, c)
\end{equation}
where $\boldsymbol{\eta} = \Phi_{\mathrm{P}}(r, c) \in \hanxiR^{d_f}$ is usually
termed Position Code in the literature \cite{he2022masked}, with the row-column coordinate
$[r, c]$ of $\mathbf{f}$ extracted from the feature tensor $\mathbf{F} \in
\hanxiR^{h_f \times w_f \times d_f}$.  The function $\Phi_{\mathrm{P}}(\cdot)$ denotes the
positional embedding process that calculates the $k$-th element of $\boldsymbol{\eta}$ as 
\begin{equation}
  \label{equ:pe}
  \eta_k =
\begin{cases}
  \mathrm{sin}(\dfrac{c}{10000^{8k/d_f}})& k\in[0,\dfrac{d_f}{4})\\
  \mathrm{cos}(\dfrac{c}{10000^{8(k-d_f/4)/d_f}})& k\in[\dfrac{d_f}{4},\dfrac{d_f}{2})\\
  \mathrm{sin}(\dfrac{r}{10000^{8(k-d_f/2)/d_f}})& k\in[\dfrac{d_f}{2},\dfrac{3d_f}{4})\\
  \mathrm{cos}(\dfrac{r}{10000^{8(k-3d_f/4)/d_f}})& k\in[\dfrac{3d_f}{4},d_f)
\end{cases}
\end{equation}
where $k \in [1, d_f]$, $r \in [1, h_f]$, $c \in [1, w_f]$.
% where $\rho$ is the quantization parameter which will be further explained in
% Sec.~\ref{subsec:swin}.
%
In this way, the whole patch feature matching process is constrained by the positional
information and the new patch feature is termed ``Position Constrained Feature'' (PCF) in
this work. The ablation study in Section~\ref{subsec:Ablation_study} verifies the merit of
this constraint. 
% Note that Equation~\ref{equ:pe} mainly follows the positional embedding method used in
% . Better position code may be obtained via a careful design of
% $\Phi_{\mathrm{P}}(\cdot)$, but that is out of the scope of this work. 

\subsubsection{Matching in the Lower Dimensional Space}
\label{subsubsec:far}
The conventional patch matching process is slow and thus unacceptable in many real-life
applications, especially in the scenario of this work where the residual generation is
only the first stage of the whole framework.  Consequently, we propose a novel algorithm
to generate the anomaly residuals faster while maintaining their discriminative property.
Firstly, the patch matching is performed in a lower-dimensional space. A Principle
Component Analysis (PCA) is conducted over the PCFs extracted from the training set and
then a PCF $\mathbf{p} \in \hanxiR^{d_f}$ is mapped to an lower-dimensional space as
\begin{equation}
  \label{equ:pca}
  \boldsymbol{\gamma} = \Psi_{\text{PCA}}(\mathbf{p}) = \mathrm{W}_{\text{PCA}}(\mathbf{p}
  - \boldsymbol{\mu}_{\text{PCA}}) \in \hanxiR^{d_l}, 
\end{equation}
where $d_l \ll d_f$ denotes the lower dimension, $W_{\text{PCA}} \in
\hanxiR^{d_l
\times d_f}$ and $\boldsymbol{\mu}_{\text{PCA}} \in \hanxiR^{d_f}$ stand for the PCA
mapping matrix and the mean feature vector respectively, $\boldsymbol{\gamma} \in
\hanxiR^{d_l}$ denotes the feature for faster patch matching. In this way, one can convert the bank $\mathcal{B}$ defined in
Eq.~\ref{equ:coreset} into its position-constrained and lower-dimensional version as
\begin{equation}
%   \resizebox{.9\hsize}{!}
%   {$
  \mathcal{B}_{raw} \xrightarrow{+\lambda_{\mathrm{P}}\boldsymbol{\eta}} 
  \mathcal{B}^{P}_{raw} \xrightarrow{\Psi_{\text{core}}(\cdot)}
  \mathcal{B}^{P} 
  \xrightarrow{\Psi_{\text{PCA}}(\cdot)} 
  \mathcal{B}^P_l.
%   $}
\end{equation}
where the operation ``$+\lambda_P\boldsymbol{\eta}_i$'' stands for the generation of PCF,
the yielded $\mathcal{B}^P_l = \{{\boldsymbol{\gamma}}^{ref}_t \in \hanxiR^{d_l} \mid
\forall t = 1, \cdots, T\}$. Then for the $i$-th ($i \in [1, 2, \cdots, h_f\cdot w_f]$)
test patch, the patch matching can be performed faster in this lower-dimensional space as  
\begin{equation}
  \label{equ:fast}
  t^{\ast} = \hanxiargmin{\forall t = 1, \cdots, T}\|\boldsymbol{\gamma}^{tst}_i -
  {\boldsymbol{\gamma}}^{ref}_t\|_{l_2},
\end{equation}
where $\boldsymbol{\gamma}^{tst}_i = \Psi_{\text{PCA}}(\mathbf{p}^{tst}_{i})$ represents the lower-dimensional PCF of the test patch.

\subsubsection{Matching with Qualified Reference Images}
Secondly, to further increase the matching speed, we propose to reduce the number of the
reference images for each test patch via an filtering stage. \emph {In this work, a test patch is only matched with the reference patches which are extracted from the qualified reference images which are ``similar'' to the test image.} To define the image similarity, let us generate the image feature of an image $\mathrm{I}$ as
\begin{equation}
\begin{tikzcd}
  \mathbf{F} \in \hanxiR^{h_f \times w_f \times d_f}
  \arrow[r, "+\lambda_P\boldsymbol{\eta}"]
   & 
  \mathbf{P} \in \hanxiR^{h_f \times w_f \times d_f} 
  \arrow[d, "\Psi_{\text{PCA}}(\cdot)"] 
  \\ 
  \boldsymbol{\Gamma} \in \hanxiR^{h_l \times w_l \times d_l}
  & 
  \mathbf{P}_l \in \hanxiR^{h_f \times w_f \times d_l}, 
  \arrow[l, "\mathrm{resize}"]
\end{tikzcd}
\end{equation}
where $\mathbf{F} = \Psi_{\mathrm{CNN}}(\mathrm{I})$ as defined in Eq.~\ref{equ:extract},
$\mathbf{P}$ denotes the feature tensor containing $h_f\cdot w_f$ PCFs, the ``resize''
operation indicates to reduce the width and height of the feature tensor via
interpolation. Then the ``flattened'' version of the image feature $\boldsymbol{\Gamma}$ writes 
\begin{equation}
  \boldsymbol{\Gamma} \to \mathrm{Flatten} \to \{\boldsymbol{\gamma}_1,
  \boldsymbol{\gamma}_2, \cdots, \boldsymbol{\gamma}_V\},
k \in [1, d_f]\end{equation}
where $V = h_l\cdot w_l$ and $h_l < h_f, ~w_l < w_f$. Now we can calculate the robust
image distance $\delta_j$ between the $j$-th ($j\in[1, 2, \cdots, N_{trn}]$) reference
image $\mathrm{I}^{ref}_j$ and the test image $\mathrm{I}^{tst}$ as 
\begin{equation}
  \label{equ:robust_dist}
  \delta_j = \Delta(\mathrm{I}^{tst}, \mathrm{I}^{ref}_j) = \sum\limits^V_{v = 1}\mathbbm{1}(v \in
  \mathcal{D}_{U})\|\boldsymbol{\gamma}^{tst}_v - \boldsymbol{\gamma}^{ref}_v\|_{l_2}
\end{equation}
where $\|\boldsymbol{\gamma}^{tst}_v - \boldsymbol{\gamma}^{ref}_v\|_{l_2}$ stands for the
patch distance between the two images in the $v$-the site, $\mathbbm{1}(\cdot)$ stands for
the indicator function, the set $\mathcal{D}_{U}$ stores the patch indexes from $1$ to $V$
except those corresponding to the top-$U$ ($U < V$) largest patch distance. Given the test-reference distances $\{\delta_1, \delta_2, \cdots, \delta_{N_{trn}}\}$, the image indexes
of ``qualified reference images'' are defined as
\begin{equation}
  \label{equ:knn}
  \resizebox{.88\hsize}{!}
  {
  $\{\delta_1, \delta_2, \cdots, \delta_{N_{trn}}\} \xrightarrow{K\texttt{-NN Indexes}}
   \mathcal{Q} = \{q_1, q_2, \cdots, q_K\}$
   }
\end{equation}
In other words, the patch matching is only performed between the patches from $\mathrm{I}^{tst}$ and
those patches belongs to the above $K$ ($K \ll N_{trn}$) nearest images. In this way, the
matching speed is further increased. 
%From another perspective, this selection operation
%can be viewed as filtering out the unrelated reference images which can also lift the
%robustness of patch matching, as practically proved in the experiment part. 

\subsubsection{The Generation Process of PosFAR}
Given a test image $\mathrm{I}^{tst}$ and a set of defect-free training images
$\{\mathrm{I}^{ref}_1, \mathrm{I}^{ref}_2, \cdots, \mathrm{I}^{ref}_{N_{trn}}\}$, the
end-to-end generation process of the proposed PosFAR can be divided into the following
four steps 
\begin{itemize}
  \item Extract the corresponding PCFs for the test image and save them into the feature
    set $\{{\mathbf{p}}^{tst}_i \in \hanxiR^{d_f} \mid \forall i = 1, \cdots, M\}$; Similarly, sample the PCFs
    of all the training images to generate the bank $\mathcal{B}^P =
    \{{\mathbf{p}}^{ref}_t \in \hanxiR^{d_f} \mid \forall t = 1, \cdots, T\}$ via
    the sampling method $\Psi_{\mathrm{core}}(\cdot)$. Meanwhile, record the training
    image index of each element of $\mathcal{B}^P$ into the set $\{j_1, j_2, \cdots,
    j_T\}$.
  \item Fit a PCA model $\Psi_{\mathrm{PCA}}(\cdot)$ based on $\mathcal{B}^P$ and generate
    the dimension-reduced feature sets $\{\boldsymbol{\gamma}^{tst}_i \in \hanxiR^{d_l}
    \mid \forall i = 1, \cdots, M\}$ (test) and $\mathcal{B}^P_l =
    \{\boldsymbol{\gamma}^{ref}_t \in \hanxiR^{d_l} \mid \forall t = 1, \cdots, T\}$
    (bank). 
  \item
    Calculate the robust distance between $\mathrm{I}^{tst}$ and all the training images
    via Eq.~\ref{equ:robust_dist} and then obtain the set of ``qualified image indexes''
    $\mathcal{Q} = \{q_1, q_2, \cdots, q_K\}$ as Eq.~\ref{equ:knn}.
  \item
    Match each test patch feature $\boldsymbol{\gamma}^{tst}_i$ with $\mathcal{B}^P_l$ via
    a faster version of Eq.~\ref{equ:fast}, which writes 
    \begin{equation}
      \label{equ:faster}
      t^{\ast} = \hanxiargmin{\forall j_t \in \mathcal{Q}}\|\boldsymbol{\gamma}^{tst}_i -
      {\boldsymbol{\gamma}}^{ref}_t\|_{l_2},
    \end{equation}
    where the constraint $j_t \in \mathcal{Q}$ indicates that the matching is only
    performed on the reference patches extracted from the qualified training images.
    Finally the proposed PosFAR feature of the $i$-th test patch is calculated as 
    \begin{equation}
    \label{equ:posfar}
      \mathbf{r}_i = \lceil \text{ABS}(\boldsymbol{\gamma}^{tst}_i -
      {\boldsymbol{\gamma}}^{ref}_{t^{\ast}}) \rceil^{\theta} \in \hanxiR^{d_f}, ~
      i\in[1, \cdots, M]
    \end{equation}
\end{itemize}
Note that each PosFAR feature $\mathbf{r}_i$, defined above represents an
image patch or ``image block'' as it is usually referred to in this paper. The anomaly
score of those image blocks are then evaluated by using the swin transformer model
introduced below.

\subsection{Train the Residual-based Swin Transformer for Block-wise Anomaly Detection}
\label{subsec:swin}

\subsubsection{Block-wise Anomaly Labels}

Encouraged by the successive pioneering work \cite{roth2022towards, zhang2022prototypical,
yang2023memseg, zhang2023destseg}, in this paper, a discriminative model is also employed
to predict the anomaly score map for test images. In the conventional ``unsupervised''
setting (as described in Sec.~\ref{subsec:supervision}), pseudo defective regions are
usually augmented onto the defect-free training images and so that the segmentation model
\cite{roth2022towards, zhang2022prototypical, yang2023memseg, zhang2023destseg} can be
trained smoothly. As the defective pixels are all artificial so the pixel-wise labels
are directly available. 

However, recall that the basic building blocks of this work are the feature residuals with
each one corresponding to an image block. We thus propose to cast the original pixel-wise
segmentation task into a block classification problem. In other words, the proposed model
in this work only predicts the anomaly label of each image block, as shown in
Fig.~\ref{fig:infer}. The yielded anomaly confidences of the blocks are then upsampled
into the pixel-wise anomaly map with the same size of the input image. Accordingly, in
this scenario, one needs to convert the conventional pixel labels into the block labels. 

Given a defective image $\mathrm{I} \in \hanxiR^{h_{\mathrm{I}} \times w_{\mathrm{I}}
\times 3}$, the associated pixel-wise label map $\mathrm{Y}^{\ast}_{\mathrm{I}} \in
\hanxiR^{h_{\mathrm{I}} \times w_{\mathrm{I}}}$ writes 
\begin{equation}
  ~ \mathrm{Y}^{\ast}_{\mathrm{I}}(r_{\mathrm{I}}, c_{\mathrm{I}}) =
  \begin{cases}
    1 & \text{anomalous pixel} \\
    -1 & \text{nominal pixel}
  \end{cases}
\end{equation}
with $r_{\mathrm{I}} \in [1, h_{\mathrm{I}}]$ and $c_{\mathrm{I}} \in [1,
w_{\mathrm{I}}]$. Then we define our block-wise label map $\mathrm{Y}^{\ast}_{f} \in
\hanxiR^{h_f \times w_f}$ as
\begin{equation}
  \label{equ:block_label}
  ~ \mathrm{Y}^{\ast}_{f}(r_f, c_f) =
  \begin{cases}
    1 & \mathlarger{\mathlarger{\sum}}\limits_{(r_{\mathrm{I}}, c_{\mathrm{I}}) \in  \mathcal{U}_{r_f,
    c_f}}\mathrm{Y}^{\ast}_{\mathrm{I}}(r_{\mathrm{I}}, c_{\mathrm{I}}) > \epsilon^{+}\rho^2 \\
    -1 & \mathlarger{\mathlarger{\sum}}\limits_{(r_{\mathrm{I}}, c_{\mathrm{I}}) \in  \mathcal{U}_{r_f,
    c_f}}\mathrm{Y}^{\ast}_{\mathrm{I}}(r_{\mathrm{I}}, c_{\mathrm{I}}) < \epsilon^{-}\rho^2\\
    \emptyset & \text{otherwise}
  \end{cases}
\end{equation}
where $\mathcal{U}_{r_f, c_f}$ denotes the pixels belonging to the image block at
coordinate $[r_f, c_f]$; $\rho = h_{\mathrm{I}}/{h_f} = w_{\mathrm{I}}/{w_f}$;
$\epsilon^{+}$ and $\epsilon^{-}$ are the two predefined thresholds determining the block
labels; when labeled as $\emptyset$, the block is ignored during training, as introduced
in Sec.~\ref{subsubsec:swin}. Fig.~\ref{fig:block_label} illustrates this block labeling
scheme. 
\begin{figure}[ht]  
  \centering
\includegraphics [width=0.4\textwidth]{block_label.pdf}
\caption{
  The block labeling strategy employed in this work. The blocks with more than
  $\epsilon^{+}\rho^2$ anomaly pixels are labeled $1$ (red) while those blocks with less than
  $\epsilon^{-}\rho^2$ are labeled $0$ (blue). The remaining blocks are labeled
  $\emptyset$ and will be ignored in the training phase.
}
\label{fig:block_label}
\end{figure}

In this work, the block-wise labels are employed for the synthetic defects in the
unsupervised setting as well as the genuine defects in the supervised setting. The
experimental results of this work verify the superiority of this labeling strategy. On the
other hand, in real-life AD tasks, one only needs to manually label image blocks rather
than pixels and thus significant reduction on annotation cost is achieved. 

\subsubsection{Swin Transformer with Focal Loss}
\label{subsubsec:swin}
As introduced above, we convert the AD task into a block-wise binary classification
problem, which is solved by using a Swin Transformer model \cite{liu2021swin}. In
specific, given a test image $\mathrm{I}^{tst} \in \hanxiR^{h_{\mathrm{I}} \times
w_{\mathrm{I}} \times 3}$, its PosFARs $\mathbf{r}_i \in \hanxiR^{d_f}, i = 1, 2, \cdots,
M$ are calculated via Equations~\ref{equ:posfar} then fed into the Swin Transformer model
as the input tokens \cite{dosovitskiyimage, liu2021swin}. 

To suit the relatively small training sets in most anomaly detection challenges
\cite{bergmann2019mvtec, mishra2021vt}, we design our Swin Transformer model with low
complexity. As shown in Fig.~\ref{fig:infer}, a linear embedding layer is firstly applied
to the PosFAR features, projecting them into a $1024$-dimensional space. Subsequently, $4$
Swin Transformer blocks are employed to realize a $32$-head self-attention within $8
\times 8$ regular windows (W-MSA) and shifted windows (SW-MSA). Finally, the tokens with
each representing an image block are classified as nominal or anomalous via a fully
connected layer. In mathematics, we have 
\begin{equation}
  p^i_{+} = \Psi_{\mathrm{Swin}}(\mathbf{r}_i), ~ \forall i \in [1, 2, \cdots, M],
\end{equation}
where $p^i_+ \in [0, 1]$ denotes the normalized anomaly confidence (of the $i$-th token)
predicted by the Swin Transformer model $\Psi_{\mathrm{Swin}}(\cdot)$

Considering that the normal image blocks usually dominate the original data distribution,
we employ the focal loss \cite{lin2017focal} to lift the importance of the anomaly class.
The focal loss used in this work writes:
\begin{equation}
  \label{equ:focal}
  \begin{split}
    \mathcal{L}_{F} = & -\dfrac{1}{|\mathcal{Z}^{-}|}\sum\limits_{i \in \mathcal{Z}^{-}}\left[ (1-\alpha)
    {p_{+}^i}^{\gamma}\mathrm{log}(1 - p^i_{+})\right] \\
    & -\dfrac{1}{|\mathcal{Z}^{+}|} \sum\limits_{i \in \mathcal{Z}^{+}}\left[ \alpha
    (1-p^i_{+})^{\gamma}\mathrm{log}(p^i_{+})\right]
  \end{split}
\end{equation} where $\mathcal{Z}^{+}$ and $\mathcal{Z}^{-}$ stands for the training
sample sets (here are transformer tokens) corresponding to defective ($+$) and defect-free
($-$) classes respectively. 

\subsubsection{Randomly Masked Residuals}
\label{subsubsec:dropout}

Different from the vanilla vision transformers \cite{dosovitskiyimage, liu2021swin,
Liu_2022_CVPR}, the input to our model is essentially \textit{feature residual vectors}.
Most conventional data augmentation methods \cite{shorten2019survey, yun2019cutmix,
yang2022image} designed for images can not be directly used in the current situation.
By contrast, inspired by the
recently proposed MAE algorithm \cite{he2022masked}, we design a simple but effective feature
augmentation approach termed ``Randomly Masked Residuals'' for achieving higher generalization
capacity. In specific, when training, each tokens $\{\mathbf{r}_1, \mathbf{r}_2, \cdots,
\mathbf{r}_M\}$ defined in Eq.~\ref{equ:posfar} is randomly ``masked'' or ``noised'' as
\begin{equation}
  \label{equ:dropout}
  \forall i, ~\mathbf{r}_i = 
  \begin{cases}
    \mathbf{0}^{\mathrm{T}} \in \hanxiR^{d_t} ~ & \tau \in [0, \alpha] \\
     \mathbf{r}_i + \kappa \frac{\|\mathbf{r}_i\|_{l_2}}{\|\mathbf{g}\|_{l_2}}\mathbf{g} ~
     & \tau \in (\alpha, 1] \\
  \end{cases}
\end{equation}
where $\tau$ is a random variable sampled from the uniform distribution $[0, 1]$; $\alpha$
is the constant controlling the frequency of the reset operation; $\mathbf{g} \in
\hanxiR^{d_f}$ denotes a Gaussian noise vector; $\kappa \in [0, 1]$ is a small constant
for merging the noise. We found this augmentation approach can effectively increase the final
performance of the proposed method, as shown in Sec.~\ref{subsec:Ablation_study}. 

\subsubsection{Off-the-shelf methods for generating fake anomalies} 
In the ``unsupervised'' setting of AD tasks, one needs to generate fake anomalies to train a
discriminative model properly. In this work, we follow the off-the-shelf fake/simulated
anomaly generation approach proposed in the MemSeg algorithm \cite{yang2023memseg}.
Readers are recommended to the original work \cite{yang2023memseg} for more details. Note
that we also employ this anomaly generation method for the supervised and
weakly-supervised settings to increase the variation of the training samples.

\subsection{Exploiting the Unlabeled Information via ResMixMatch}
\label{subsec:mixmatch}

\subsubsection{The Weaker Labels with Trivial Labeling Cost}
Recent researches on the ``supervised'' AD tasks \cite{ding2022catching,
zhang2022prototypical, yao2022explicit, bovzivc2021mixed-KolektorSDD2} have demonstrated
the benefit of exploiting the real defective samples. Nonetheless, this benefit is
obtained at the cost of much longer annotation time. The block-wise label proposed in this
paper can reduce the cost to some extent while there is still a large room for improvement. 

To further reduce the annotation cost, we introduce three types of anomaly labels which
are much ``cheaper'' than the block-wise ones. As depicted in Fig.~\ref{fig:weaker}. the
proposed weak labels include the ``rotated bounding-boxes'' (left), the ``axis-aligned
bounding-boxes'' (middle) and the ``image-level labels'' (right). From the figure we can
see that the bounding box labels are the minimal rectangles covering the whole defective
region, with or without rotation. On the other hand, the image-level label just represents
the defective status of the image. 
These weak labels only requires the annotators input a few ($1$ to $4$) clicks on the
image, which is much more efficient than the conventional pixel labels and the
proposed block labels. 

\begin{figure}[ht]  
  \centering
\includegraphics [width=0.45\textwidth]{weaker_labels.pdf}
\caption{The three types of weak labels employed in this work. From left to right: the
  ``rotated bounding-boxes'' (left), the ``axis-aligned bounding-boxes'' (middle) and the
  ``image-level labels'' (right). The lower part of each column illustrates the block-wise
  label converting operation for the associated weak label.}
\label{fig:weaker}
\end{figure}

In the block-based framework of this work, one needs to convert the weaker labels into the
block-wise annotations for model training. The lower part of Fig.~\ref{fig:weaker}
illustrates the label converting processes for the three kinds of weak labels. In a
nutshell, for the bounding-box-based labels, we consider the outside region of the
bounding boxes as normal while the inside region are treated as ``unknown''.  To formally
define the label conversion, let us first introduce the ``Overlapping Ratio'' function
$\Psi_{\mathrm{OR}}(\text{A}, \text{B})$ as
\begin{equation}
  \Psi_{\mathrm{OR}}(\text{A}, \text{B}) = area(intersection(\text{A}, \text{B})) /
  area(\text{A}).
\end{equation}
where A and B are two arbitrary regions on the image; the operations $area(\cdot)$ and
$intersection(\cdot, \cdot)$ are both conducted in the {\bf image pixel space}. Then the
label conversion is defined as   
\begin{equation}
  \label{equ:block_label_semi}
  ~ \mathrm{Y}^{\ast}_{f}(r_f, c_f) =
  \begin{cases}
    {-}1 & \Psi_{\mathrm{OR}}(\text{blk}_{[r_f, c_f]}, \text{bbox}) < 0.5\\
    \emptyset & \text{otherwise}, 
  \end{cases}
\end{equation}
where ``$\text{blk}_{[r_f, c_f]}$'' denotes the image block at the $r_f$-th row and
$c_f$-th column in the feature space; ``bbox'' stands for the manually labeled
bounding-box. On the contrary, the conversion for the image-level labels are much simpler:
all the image blocks are set ``unknown'' for a defective image while those of a
defect-free image are all labeled $-1$.

Note that the proposed weak labels are partially inspired by the pioneering works
\cite{Tabernik2019JIM-KolektorSDD, bovzivc2021mixed-KolektorSDD2} that also employ
bounding boxes to annotate defective parts. However, those bounding boxes consider {\bf all} the
inside pixels as anomalies and thus usually lead to significant label ambiguities. In
contrast, we uses the bounding box to annotate the normal region and leave other
blocks as {\bf unknown}. This labeling strategy is less misleading and the unknown region
can be successfully exploited by the semi-supervised learning scheme introduced below.    

\subsubsection{Exploiting the Unlabeled blocks in a Semi-Supervised Manner}

As introduced above, the proposed weaker labels can achieve very efficient annotation
processes. However, they arise another difficulty in training: An unignorable portion of
the image blocks are unlabeled and no block is labeled as ``defective''.
%
Fortunately, this semi-supervised situation is highly well studied in the machine learning
literature \cite{zhu2009introduction, berthelot2019mixmatch, berthelot2019remixmatch,
sohn2020fixmatch, wang2023freematch}. In this work, we borrow the main concept of the
MixMatch method \cite{berthelot2019mixmatch} into the learning process of a Swin
Transformer model. The novel semi-supervised learning algorithm, termed ``ResMixMatch'',
is summarized in Algorithm~\ref{alg:mixmatch}. 

\input{mixmatch_alg}

From the algorithm we can see that, the proposed ResMixMatch algorithm only shares the
high-level concept of data-mixing with MixMatch \cite{berthelot2019mixmatch}. Besides the
replacement of images with residuals, our ResMixMatch differentiates from MixMatch on the
following three factors.
\begin{itemize}
\item
    Different from MixMatch that treats every sample independently, in ResMixMatch, all
    the PosFAR features are related. The Swin Transformer model effectively links the
    PosFARs from the same image via the self-attention mechanism and their anomaly
    confidences are then predicted dependently on each other. From the perspective of
    semi-supervised learning, the labels of the ``unknown'' blocks are estimated not only
    by the mixing-matching strategy but also based on the neighboring information. In this
    way, the estimation becomes more reliable.
%     to their original image positions ($[r, c]$) and image index. When performing the
%     Swin Transformer $\Psi_{\mathrm{Swin}}(\cdot)$, the tokens and the corresponding
%     labels from the same image are reorganized into PCR tensors and label maps, as shown
%     in step-$2$ and step-$6$ in Algorithm~\ref{alg:mixmatch}. In this way, one can sufficiently
%     use the self-attention mechanism of transformers to achieve higher generalization
%     capacity.  
\item 
    A novel augmentation method \emph{i.e.}, the Randomly Masked Residuals defined in
    Equation~\ref{equ:dropout} is employed for sample generation. The new augmentation
    methods are carefully designed to suit residual features and thus increase the
    recognition accuracy according to the experiment. 
\item
    Instead of the conventional cross-entropy loss used in \cite{berthelot2019mixmatch},
    we employ the focal loss \cite{lin2017focal} for the imbalanced label distribution in
    AD tasks.
\end{itemize}

In practice, the weakly-supervised Swin Transformer model is firstly pre-trained in the
unsupervised condition with genuine normal images and synthetic anomalies. Then we
fine-tune the model on the genuine defective samples with weak labels (determined by the
bounding-boxes or image tags) by using ResMixMatch. Usually significant performance
improvement can be obtained thanks to the successful exploitation of the unlabeled blocks,
according to the experimental result of this work.

\subsubsection{Overview of the training process}

In summary, the whole training procedure of our WeakREST is depicted in
Figure~\ref{fig:train}.  In practice, the full-supervision part (shown in blue) is adopted
for the supervised setting as well as the ``unsupervised'' setting where simulated
anomalies are generated.  In the semi-supervised setting, both the semi-supervision part
(red) and the full-supervision part (blue) are employed to guarantee high performances.
Note that this is not against to our original motivation of reducing the annotation effort
because one can always use the synthetic defects with no labeling effort.  

\begin{figure*}[ht]  
  \centering
\includegraphics [width=0.95\textwidth]{training.pdf}
\caption{
  The overview of the training process of WeakREST. Note that in the unsupervised and
  supervised settings, only the lower part (shown in blue) is used and the red part,
  \emph{i.e.}, the semi-supervision is leveraged in the semi-supervised setting. Better
  view in color. 
}
\label{fig:train}
\end{figure*}

\subsection{Foreground reweighing strategy}

% \subsection{Implementation Details}
% The AdamW \cite{loshchilovdecoupled} optimizer with the weight decay of $0.05$ is used for
% transformer training and the exponential moving average (EMA) \cite{haynes2012exponential}
% trick is adopted to smooth the parameters for the final model. 


% \subsubsection{Bagging over sliding Swin Transformers} 
% \label{subsubsec:bagging}

% The Swin Transformer is adopted as the backbone of our deep learning model with the PCRs
% as its input features, rather than normal images. Follow the conventional ViT
% % way
% \cite{dosovitskiyimage, liu2021swin, Liu_2022_CVPR}, the collection of PCRs
% $\hat{\mathbf{R}}$ is firstly partitioned into several ``feature patches''
% over the ``Row-Column'' plane. Given the pre-defined patch size $\rho$, the flattened
% transformer tokens are stored in the token tensor 
% \begin{equation}
%   \label{equ:tensor}
%   \mathbf{T} \in \hanxiR^{h_t \times w_t \times d_t}, 
% \end{equation}
% with the row number $h_t = {h_f}/{\rho}$, column number $w_t  = {w_f}/{\rho}$ and the channel
% dimension $d_t = d\rho^2$. Note that here every token vector $\mathrm{t} \in
% \hanxiR^{d_t}$ geometrically corresponds to a $(h_\mathrm{I}\rho/{h_t}) \times
% (w_\mathrm{I}\rho/w_t)$ image-pixel block on the image input of $\Psi_{\mathrm{CNN}}$. 

% As it is illustrated in Figure~\ref{fig:infer}, a number of ``sub-tensors'' are extracted from
% $\mathbf{T}$ in a sliding-window fashion. Let us define the square windows sliding on the
% Row-Column plane as: 
% \[
%   \mathbf{w} = [r^t, c^t, \mu]^{\mathrm{T}} 
% \]
% where $[r^t, c^t]$ stands for the coordinate of the window's top-left corner; $\mu$ is
% the size of the square window; $c^t \in [0, w_t - \mu)$ and $r^t \in [0, h_t -
% \mu)$. A sub-tensor is sliced from $\mathbf{T}$ according to $\mathbf{w}$ as:
% \begin{equation}
%   \label{equ:input_tensor}
%   \mathbf{T}_{\mathbf{w}} = \mathbf{T}[r^t : r^t + \mu - 1, c^t : c^t + \mu -1, :] \in
%   \hanxiR^{\mu \times \mu \times d_t}.
% \end{equation}
% The sub-tensor is then fed into the Swin Transformer model to generate the prediction map
% as
% \begin{equation}
%   \Psi_{\mathrm{Swin}}(\mathbf{T}_{\mathbf{w}}) = \Theta_{\mathbf{w}} \in \hanxiR^{\mu
%   \times \mu}.
% \end{equation}
% Note that the output of $\Psi_{\mathrm{Swin}}(\cdot)$ for each token is actually a
% $2$-D vector, we directly copy the confidences corresponding to the anomaly class to
% $\Theta_{\mathbf{w}}$. 

% In specific, given a pre-defined sampling step $s$ and a fixed size $\mu$, one can
% generates $Q$ square sliding windows $\{\mathbf{w}_1, \mathbf{w}_2, \cdots,
% \mathbf{w}_Q\}$ and the corresponding prediction maps $\{\Theta_{\mathbf{w}_1},
% \Theta_{\mathbf{w}_2}, \cdots, \Theta_{\mathbf{w}_Q}\}$.  Now each element of the final
% prediction map $\Theta \in \hanxiR^{h_t \times w_t}$ for the holistic tensor
% $\mathbf{T}$ can be calculated as 
% \begin{equation}
%   \Theta(r,c) =
%   \frac{1}{|\mathcal{N}_{r,c}|}\sum_{i\in\mathcal{N}_{r,c}}\Theta_{\mathbf{w}_i}(r - r^t_i,
%   c - c^t_i)
% \end{equation}
% where $r \in [0, h_t)$ and $c \in [0, w_t)$ are the row and column indexes of the map
% element; $\mathcal{N}_{r,c}$ stands for the set of sliding windows overlapping with
% location $(r, c)$; $|\cdot|$ represents the set cardinality; the subtractions $r - r^t_i$
% and $c - c^t_i$ are the coordinate translation operations. 

% From the perspective of machine learning, the
% ano\-maly score for each token $\mathrm{t}_{r,
% c}$ is achieved by aggregating the outputs of $|\mathcal{N}_{r,c}|$ Swin Transformers
% which are fed with different PCRs. In this way, the noise could be averaging out from the
% final prediction. In this paper, with a gentle generalization to the original definition,
% we term this sliding-aggregating strategy as Swin Transformer ``Bagging'' (Bootstrap
% Aggregating) \cite{breiman1996bagging}. The ablation study in Section~

% One then can build the memory bank following the method proposed in \cite{roth2022towards}
% as 
% \begin{equation}
%   \hat{\mathcal{M}} = \Psi(\mathcal{F}_{\mathrm{trn}}) = \{\hat{\mathbf{m}}_t \in
%   \hanxiR^{d_f} \mid t = 1, 2, \cdots, T\}
% \end{equation}
% where $\hat{\mathcal{M}}$ is the memory bank containing $T$ PCFs ($\hat{\mathbf{m}}_t,
% \forall t$), $\Psi(\cdot)$ represents the ``coreset'' sampling scheme of PatchCore
% \cite{roth2022towards}, $\hat{\mathcal{F}}_{\mathrm{trn}} = \{\hat{\mathbf{f}}_i \in
% \hanxiR^{d_f} \mid i = 1, 2, \cdots, N\}$ denotes the original feature set consisting
% $N$ PCFs, which are extracted from all the normal images for training.
% %
% Finally, given a test PCF $\hat{\mathbf{f}}_i$, the corresponding ``Posi\-tion
% cons\-trained Residual'' (PCR) can be calculated in the PatchCore manner
% \cite{roth2022towards} as 
% \begin{equation}
%   \label{equ:pcr}
%   \hat{\mathbf{r}}_i = \mathcal{S}\left(\hat{\mathbf{f}}_i - \hanxiargmin{\forall \hat{\mathbf{m}}_t \in
%   \hat{\mathcal{M}}}\|\hat{\mathbf{f}}_i - \hat{\mathbf{m}}_t\|_{l_2}\right) \in \hanxiR^{d_f},
% \end{equation}
% with the element-wise square function $\mathcal{S}(\cdot)$ defined as 
% \begin{equation}
% \label{equ:square}
% \mathcal{S}\left([x_1, x_2, \cdots, x_{d_f}]^{\mathrm{T}}\right) = [x^2_1, x^2_2, \cdots, x^2_{d_f}]^{\mathrm{T}}.
% \end{equation}
% Compared with the absolute values of the tensor difference employed in
% \cite{zhang2022prototypical}, the yielded residual vector $\hat{\mathbf{r}}_i$ in Equation
% \ref{equ:pcr} is more sparse and this ``feature-selection'' property empirically benefits
% the following training process, as it is shown in Section~\ref{subsec:Ablation_study}.
% %
% According to Equations~\ref{equ:extract} and \ref{equ:pcr}, we can generate $M$ PCRs from a test
% image $\mathrm{I}$ as shown in Figure~\ref{fig:infer}. The $M$ PCRs are then reorganized to form
% the PCR tensor $\hat{\mathbf{R}} \in \hanxiR^{h_f \times w_f \times d_f}$. 

% A long-standing dilemma existing in anomaly detection is whether to involve the real-world
% defective samples in the training stage. Different choices lead to two main types of AD
% tasks, \emph{i.e.}, the mainstream ``unsupervised'' setting
% \cite{defard2021padim,roth2022towards,lei2023pyramidflow,hou2021divide,bergmann2022beyond,liu2023diversity}

% To strike the balance between the annotation time and model performances, we propose to
% label the realistic defects using bounding boxes which require much less annotation labor
% compared with the commonly-used pixel-wise labels in the ``supervised'' setting
% \cite{ding2022catching, zhang2022prototypical, yao2022explicit,
% bovzivc2021mixed-KolektorSDD2}. However, as shown in Figure~\ref{fig:high_level}, the
% bounding boxes, that jointly cover all the anomaly pixels on the image, can only guarantee
% the correctness of the negative (normal) label of the outside region of the boxes.  The
% pixel labels inside the box union are unknown. 

% In the semi-supervised scenario, the pixel labels are estimated by the bounding boxes.  In
% particular, the pixels outside the union of boxes are labeled as $0$ (normal) and other
% pixels are labeled as ${-}1$ (unknown). So in this scenario $\mathrm{Y}^{\ast}_{P}
% \in \mathbb{Z}^{\mu \times \mu}_2$ with $\mathrm{Y}^{\ast}_{P}(r, c) \in
% \{0~\text{(normal)},$
% $ {-}1~\text{(unknown)}\}$. Similarly to Equation~\ref{equ:block_label}, the
% block-wise semi-supervision is defined as
% where $\upsilon$ is the threshold for determining whether the label of the block is
% unknown.


